A Python Extension to Simulate Petri nets in Process Mining

The capability of process mining techniques in providing extensive knowledge and insights into business processes has been widely acknowledged. Process mining techniques support discovering process models as well as analyzing process performance and bottlenecks in the past executions of processes. However, process mining tends to be "backward-looking" rather than "forward-looking" techniques like simulation. For example, process improvement also requires "what-if" analyses. In this paper, we present a Python library that uses an event log to directly generate a simulated event log, with additional options for end-users to specify the duration of activities and the arrival rate. Since the generated simulation model is supported by historical data (event data)and it is based on the Discrete Event Simulation (DES) technique, the generated event data is similar to the behavior of the real process.

==> Reference.tex <==

@incollection{DBLP:series/ihis/Aalst15,
  author    = {Wil M. P. van der Aalst},
  title     = {Business Process Simulation Survival Guide},
  booktitle = {Handbook on Business Process Management 1, Introduction, Methods,
               and Information Systems, 2nd Ed.},
  publisher = {Springer},
  pages     = {337--370},
  year      = {2015}
}

@inproceedings{DBLP:conf/caise/Aalst10,
  author    = {Wil M. P. van der Aalst},
  title     = {Business Process Simulation Revisited},
  booktitle = {Enterprise and Organizational Modeling and Simulation - 6th International
               Workshop, {EOMAS} 2010},
  pages     = {1--14},
  year      = {2010}
}

@book{sterman2000business,
  title={Business dynamics: systems thinking and modeling for a complex world},
  author={Sterman, John D},
  publisher={McGraw-Hill},
  year={2000}
}

@inproceedings{DBLP:conf/scsc/Aalst18,
  author    = {Wil M. P. van der Aalst},
  title     = {Process mining and simulation: a match made in heaven!},
  booktitle = {Proceedings of the 50th Computer Simulation Conference, SummerSim
               2018, Bordeaux, France, July 09-12, 2018},
  pages     = {4:1--4:12},
  publisher = {{ACM}},
  year      = {2018},
  url       = {http://dl.acm.org/citation.cfm?id=3275386},
  timestamp = {Thu, 06 Sep 2018 10:11:18 +0200},
  biburl    = {https://dblp.org/rec/conf/scsc/Aalst18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@techreport{meadows2008thinking,
  title={Thinking in Systems: A Primer, edited by: Wright, D., Earthscan, London, 218},
  author={Meadows, DH},
  year={2008},
  institution={ISBN 978-1-84407-726-7}
}

@inproceedings{rosenberg2015system,
  title={A System Dynamics Model for Business Process Change Projects},
  author={Rosenberg, Zuzana and Riasanow, Tobias and Krcmar, Helmut},
  booktitle={International Conference of the System Dynamics Society},
  pages={1--27},
  year={2015}
}


@article{sterman2002all,
  title= {{All Models are Wrong: Reflections on Becoming a Systems Scientist}},
  author={Sterman, John D},
  journal={System Dynamics Review: The Journal of the System Dynamics Society},
  volume={18},
  number={4},
  pages={501--531},
  year={2002},
  publisher={Wiley Online Library}
}





@book{DBLP:books/sp/Aalst16,
  author    = {Wil M. P. van der Aalst},
  title     = {Process mining - data science in action, Second Edition},
  publisher = {Springer},
  year      = {2016},

  isbn      = {978-3-662-49850-7}
}
%  doi       = {10.1007/978-3-662-49851-4},


@article{DBLP:journals/is/RozinatMSA09,
  author    = {Anne Rozinat and
               R. S. Mans and
               Minseok Song and
               Wil M. P. van der Aalst},
  title     = {Discovering simulation models},
  journal   = {Inf. Syst.},
  volume    = {34},
  number    = {3},
  pages     = {305--327},
  year      = {2009},
  doi       = {10.1016/j.is.2008.09.002},
}




@article{sterman2002system,
  title={{System Dynamics: Systems Thinking and Modeling for a Complex World}},
  author={Sterman, John},
  year={2002},
  publisher={Massachusetts Institute of Technology. Engineering Systems Division}
}

@proceedings{DBLP:conf/otm/2016,
  editor    = {Christophe Debruyne and
               Herv{\'{e}} Panetto and
               Robert Meersman and
               Tharam S. Dillon and
               eva K{\"{u}}hn and
               Declan O'Sullivan and
               Claudio Agostino Ardagna},
  title     = {On the Move to Meaningful Internet Systems: {OTM} 2016 Conferences
               - Confederated International Conferences: CoopIS, C{\&}TC, and
               {ODBASE} 2016, Rhodes, Greece, October 24-28, 2016, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {10033},
  year      = {2016},
  isbn      = {978-3-319-48471-6},
  timestamp = {Fri, 02 Nov 2018 09:45:39 +0100},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{hornix2007performance,
  title={Performance analysis of business processes through process mining},
  author={Hornix, Peter TG},
  journal={Master's Thesis, Eindhoven University of Technology},
  year={2007},
  publisher={Citeseer}
}

@article{houghton2015advanced,
  title={Advanced data analytics for system dynamics models using PySD},
  author={Houghton, James and Siegel, Michael},
  journal={revolution},
  volume={3},
  pages={4},
  year={2015}
}


@article{DBLP:journals/dss/SuriadiOAH15,
  author    = {Suriadi Suriadi and
               Chun Ouyang and
               Wil M. P. van der Aalst and
               Arthur H. M. ter Hofstede},
  title     = {Event interval analysis: Why do processes take time?},
  journal   = {Decision Support Systems},
  volume    = {79},
  pages     = {77--98},
  year      = {2015},
  timestamp = {Wed, 14 Nov 2018 10:35:12 +0100},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{an2005developing,
  title={On developing system dynamics model for business process simulation},
  author={An, Lianjun and Jeng, Jun-Jang},
  booktitle={Proceedings of the 37th conference on Winter simulation},
  pages={2068--2077},
  year={2005},
  organization={Winter Simulation Conference}
}


@article{houghton2015advanced,
  title={Advanced data analytics for system dynamics models using PySD},
  author={Houghton, James and Siegel, Michael},
  journal={revolution},
  volume={3},
  pages={4},
  year={2015}
}

@proceedings{DBLP:conf/scsc/2018,
  title     = {Proceedings of the 50th Computer Simulation Conference, SummerSim
               2018, Bordeaux, France, July 09-12, 2018},
  publisher = {{ACM}},
  year      = {2018},
}

@inproceedings{duggan2006comparison,
  title={A Comparison of {{P}etri} Net and System Dynamics Approaches for Modelling Dynamic Feedback Systems},
  author={Duggan, James},
  booktitle={24th International Conference of the Systems Dynamics Society},
  year={2006}
}




@article{DBLP:journals/corr/abs-1811-00062,
  author    = {Niek Tax and
               Irene Teinemaa and
               Sebastiaan J. van Zelst},
  title     = {An Interdisciplinary Comparison of Sequence Modeling Methods for Next-Element
               Prediction},
  journal   = {CoRR},
  volume    = {abs/1811.00062},
  year      = {2018},
  archivePrefix = {arXiv},
  eprint    = {1811.00062}
}







@article{ghasemi2012normality,
  title={Normality tests for statistical analysis: a guide for non-statisticians},
  author={Ghasemi, Asghar and Zahediasl, Saleh},
  journal={International journal of endocrinology and metabolism},
  volume={10},
  number={2},
  pages={486},
  year={2012},
  publisher={Kowsar Medical Institute}
}
@article{razali2011power,
  title={Power comparisons of Shapiro-Wilk, Solmogorov-Smirnov, lilliefors and anderson-darling tests},
  author={Razali, Nornadiah Mohd and Wah, Yap Bee and others},
  journal={Journal of statistical modeling and analytics},
  volume={2},
  number={1},
  pages={21--33},
  year={2011}
}

@book{pruyt2013small,
  title={Small system dynamics models for big issues: Triple jump towards real-world complexity},
  author={Pruyt, Erik},
  year={2013},
  publisher={TU Delft Library}
}





@article{DBLP:journals/widm/AalstAD12,
  author    = {Wil M. P. van der Aalst and
               Arya Adriansyah and
               Boudewijn F. van Dongen},
  title     = {Replaying history on process models for conformance checking and performance
               analysis},
  journal   = {Wiley Interdiscip. Rev. Data Min. Knowl. Discov.},
  volume    = {2},
  number    = {2},
  pages     = {182--192},
  year      = {2012}
}

@inproceedings{DBLP:conf/otm/DongenCA08,
  author    = {Boudewijn F. van Dongen and
               R. A. Crooy and
               Wil M. P. van der Aalst},
  title     = {Cycle Time Prediction: When Will This Case Finally Be Finished?},
  booktitle = {On the Move to Meaningful Internet Systems: {OTM} 2008, {OTM} 2008
               Confederated International Conferences, CoopIS, DOA, GADA, IS, and
               {ODBASE} 2008, Monterrey, Mexico, November 9-14, 2008, Proceedings,
               Part {I}},
  pages     = {319--336},
  year      = {2008},
  doi       = {10.1007/978-3-540-88871-0\_22}
}



@inproceedings{ratzer2003cpn,
  author    = {Anne V. Ratzer and
               Lisa Wells and
               Henry Michael Lassen and
               Mads Laursen and
               Jacob Frank Qvortrup and
               Martin Stig Stissing and
               Michael Westergaard and
               S{\o}ren Christensen and
               Kurt Jensen},
  title     = {{CPN} Tools for Editing, Simulating, and Analysing Coloured {P}etri
               Nets},
  booktitle = {Applications and Theory of {P}etri Nets 2003, 24th International Conference,
               {ICATPN} 2003, Eindhoven, The Netherlands, June 23-27, 2003, Proceedings},
  pages     = {450--462},
  year      = {2003},
  doi       = {10.1007/3-540-44919-1\_28}
}

@book{DBLP:books/daglib/0023756,
  author    = {Kurt Jensen and
               Lars Michael Kristensen},
  title     = {Coloured {P}etri Nets - Modelling and Validation of Concurrent Systems},
  publisher = {Springer},
  year      = {2009},
  doi       = {10.1007/b95112},
  isbn      = {978-3-642-00283-0}
}



@article{DBLP:journals/dke/AugustoCDRB18,
  author    = {Adriano Augusto and
               Raffaele Conforti and
               Marlon Dumas and
               Marcello {La Rosa} and
               Giorgio Bruno},
  title     = {Automated discovery of structured process models from event logs:
               The discover-and-structure approach},
  journal   = {Data Knowl. Eng.},
  volume    = {117},
  pages     = {373--392},
  year      = {2018},
 }


@book{DBLP:books/sp/CarmonaDSW18,
  author    = {Josep Carmona and
               Boudewijn F. van Dongen and
               Andreas Solti and
               Matthias Weidlich},
  title     = {Conformance Checking - Relating Processes and Models},
  publisher = {Springer},
  year      = {2018},
  doi       = {10.1007/978-3-319-99414-7},
  isbn      = {978-3-319-99413-0}
}

@inproceedings{DBLP:conf/bpm/LeemansFA14,
  author    = {Sander J. J. Leemans and
               Dirk Fahland and
               Wil M. P. van der Aalst},
  title     = {Process and Deviation Exploration with Inductive Visual Miner},
  booktitle = {Proceedings of the {BPM} Demo Sessions 2014 Co-located with the 12th
               International Conference on Business Process Management {(BPM} 2014),
               Eindhoven, The Netherlands, September 10, 2014},
  pages     = {46},
  year      = {2014}
}


@inproceedings{DBLP:conf/bpm/MannhardtLR15,
  author    = {Felix Mannhardt and
               Massimiliano de Leoni and
               Hajo A. Reijers},
  title     = {The Multi-perspective Process Explorer},
  booktitle = {Proceedings of the {BPM} Demo Session 2015 Co-located with the 13th
               International Conference on Business Process Management {(BPM} 2015),
               Innsbruck, Austria, September 2, 2015},
  pages     = {130--134},
  year      = {2015}
}

@inproceedings{dees2017enhancing,
  title={Enhancing process models to improve business performance: a methodology and case studies},
  author={Dees, Marcus and de Leoni, Massimiliano and Mannhardt, Felix},
  booktitle={OTM Confederated International Conferences" On the Move to Meaningful Internet Systems"},
  pages={232--251},
  year={2017},
  organization={Springer}
}




@article{DBLP:journals/corr/TaxVRD16,
  author    = {Niek Tax and
               Ilya Verenich and
               Marcello La Rosa and
               Marlon Dumas},
  title     = {Predictive Business Process Monitoring with {LSTM} Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1612.02130},
  year      = {2016},
  archivePrefix = {arXiv},
  eprint    = {1612.02130}
}








@article{DBLP:journals/accs/DworzanskiL13,
  author    = {Leonid W. Dworzanski and
               Irina A. Lomazova},
  title     = {{CPN} tools-assisted simulation and verification of nested {{P}etri} nets},
  journal   = {Automatic Control and Computer Sciences},
  volume    = {47},
  number    = {7},
  year      = {2013}
}


@misc{ wiki:xxx,
    author = "{Wikipedia contributors}",
    title = "Comparison of system dynamics software --- {Wikipedia}{,} The Free Encyclopedia",
    year = "2019",
    howpublished = "\url{https://en.wikipedia.org/w/index.php?title=Comparison_of_system_dynamics_software&oldid=879077628}",
    note = "[Online; accessed 27-February-2019]"

}



@article{DBLP:journals/dke/RozinatWAHF09,
  author    = {Anne Rozinat and
               Moe Thandar Wynn and
               Wil M. P. van der Aalst and
               Arthur H. M. ter Hofstede and
               Colin J. Fidge},
  title     = {Workflow simulation for operational decision support},
  journal   = {Data Knowl. Eng.},
  volume    = {68},
  number    = {9},
  pages     = {834--850},
  year      = {2009},
  doi       = {10.1016/j.datak.2009.02.014}
}







@article{Teinemaa:2019:OPP:3319626.3301300,
  author    = {Irene Teinemaa and
               Marlon Dumas and
               Marcello La Rosa and
               Fabrizio Maria Maggi},
  title     = {Outcome-Oriented Predictive Process Monitoring: Review and Benchmark},
  journal   = {{TKDD}},
  volume    = {13},
  number    = {2},
  pages     = {17:1--17:57},
  year      = {2019},
  doi       = {10.1145/3301300}
}









@article{van2012process,
  title={Process Mining Put into Context},
  author={Wil M. P. van der Aalst and S. dustdar},
  journal={IEEE Internet Computing},
  year={2012},
  volume={16},
  pages={82-86}
}



@article{DBLP:journals/is/LeoniAD16,
  author    = {Massimiliano de Leoni and
               Wil M. P. van der Aalst and
               Marcus Dees},
  title     = {A general process mining framework for correlating, predicting and
               clustering dynamic behavior based on event logs},
  journal   = {Inf. Syst.},
  volume    = {56},
  pages     = {235--257},
  year      = {2016},
  doi       = {10.1016/j.is.2015.07.003}
}




@article{DBLP:journals/sttt/RozinatMSA08,
  author    = {Anne Rozinat and
               R. S. Mans and
               Minseok Song and
               Wil M. P. van der Aalst},
  title     = {Discovering colored {P}etri nets from event logs},
  journal   = {{STTT}},
  volume    = {10},
  number    = {1},
  pages     = {57--74},
  year      = {2008},
  doi       = {10.1007/s10009-007-0051-0}
}


@misc{https://doi.org/10.4121/uuid:5f3067df-f10b-45da-b98b-86ae4c7a310b,
  doi = {10.4121/UUID:5F3067DF-F10B-45DA-B98B-86AE4C7A310B},

  author = {{Van Dongen, B.F. (Boudewijn)}},
  keywords = {000 Computer science, knowledge & systems, Business Process Intelligence (BPI), 0806 - Information Systems, 1503 - Business and Management},
  language = {en},
  title = {BPI Challenge 2017},
  publisher = {Eindhoven University of Technology},
  year = {2017}
}

@misc{ https://doi.org/10.4121/uuid:3926db30-f712-4394-aebc-75976070e91f ,
  doi = {10.4121/uuid:3926db30-f712-4394-aebc-75976070e91f },

  author = {{Van Dongen, B.F. (Boudewijn)}},
  keywords = {000 Computer science, knowledge & systems, Business Process Intelligence (BPI), 0806 - Information Systems, 1503 - Business and Management},
  language = {en},
  title = {BPI Challenge 2012},
  publisher = {Eindhoven University of Technology},
  year = {2012}
}








@article{powers2011evaluation,
  title={Evaluation: from precision, recall and F-measure to ROC, informedness, markedness and correlation},
  journal = {Journal of Machine Learning Technologies},
  author={Powers, David Martin},
  volume = 2,
  issue = 1,
  pages = {37--63},
  year={2011},
  publisher={Bioinfo Publications}
}


@inproceedings{DBLP:conf/otm/PourbafraniZA19,
  author    = {Mahsa Pourbafrani and
               Sebastiaan J. van Zelst and
               Wil M. P. van der Aalst},
  title     = {Scenario-Based Prediction of Business Processes Using System Dynamics},
  booktitle = {On the Move to Meaningful Internet Systems: {OTM} 2019 Conferences
               - Confederated International Conferences: CoopIS, ODBASE, C{\&}TC
               2019, Rhodes, Greece, October 21-25, 2019, Proceedings},
  pages     = {422--439},
  year      = {2019},
 
  url       = {https://doi.org/10.1007/978-3-030-33246-4\_27},
  doi       = {10.1007/978-3-030-33246-4\_27},
  timestamp = {Wed, 16 Oct 2019 10:22:23 +0200},
  biburl    = {https://dblp.org/rec/conf/otm/PourbafraniZA19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{MahsaBIS,
  author    = {Mahsa Pourbafrani and
               Sebastiaan J. van Zelst and
               Wil M. P. van der Aalst},
  title     = {Supporting Automatic System Dynamics Model Generation for Simulation
               in the Context of Process Mining},
  booktitle = {Business Information Systems - 23rd International Conference, {BIS}
               2020, Colorado Springs, CO, USA, June 8-10, 2020, Proceedings},
  pages     = {249--263},
  year      = {2020},

  url       = {https://doi.org/10.1007/978-3-030-53337-3\_19},
  doi       = {10.1007/978-3-030-53337-3\_19},
  timestamp = {Fri, 24 Jul 2020 14:16:33 +0200},
  biburl    = {https://dblp.org/rec/conf/bis/PourbafraniZA20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{mahsaToolPMSD,
  author    = {Mahsa Pourbafrani and
               Wil M. P. van der Aalst},
  title     = {{PMSD}: Data-Driven Simulation in Process Mining },
  booktitle = {Proceedings of the Dissertation Award, Doctoral Consortium, and Demonstration
               Track at {BPM} 2020 co-located with 18th International Conference
               on Business Process Management, {BPM} 2020},
  pages     = {},
  year      = {2020},
  
  url       = {},
  timestamp = {{},
  biburl    = {},
}
}



@inproceedings{610,
	title = {Developing System Dynamics Models from Causal Loop Diagrams},
	year = {2004},
	booktitle= {Proceedings of the 22nd International Conference of the System Dynamics Society. Oxford, Great Britain, July 25-29, 2004},
	author = {T. Binder and A. Vox and S. Belyazid and H. Haraldsson and M. Svensson}
}



@article{schober2018correlation,
  title={Correlation coefficients: appropriate use and interpretation},
  author={Schober, Patrick and Boer, Christa and Schwarte, Lothar A},
  journal={Anesthesia \& Analgesia},
  volume={126},
  number={5},
  pages={1763--1768},
  year={2018},
  publisher={Wolters Kluwer}
}

@inproceedings{DBLP:conf/ihsi/PourbafraniZA20,
  author    = {Mahsa Pourbafrani and
               Sebastiaan J. van Zelst and
               Wil M. P. van der Aalst},
  title     = {Supporting Decisions in Production Line Processes by Combining Process
               Mining and System Dynamics},
  booktitle = {Intelligent Human Systems Integration 2020 - Proceedings of the 3rd
               International Conference on Intelligent Human Systems Integration
               {(IHSI} 2020): Integrating People and Intelligent Systems, February
               19-21, 2020, Modena, Italy},
  pages     = {461--467},
  year      = {2020},

  url       = {https://doi.org/10.1007/978-3-030-39512-4\_72},
  doi       = {10.1007/978-3-030-39512-4\_72},
  timestamp = {Mon, 27 Jan 2020 11:16:31 +0100},
  biburl    = {https://dblp.org/rec/conf/ihsi/PourbafraniZA20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
  }

@article{DBLP:journals/csur/EslingA12,
  author    = {Philippe Esling and
               Carlos Ag{\'{o}}n},
  title     = {Time-series data mining},
  journal   = {{ACM} Comput. Surv.},
  volume    = {45},
  number    = {1},
  pages     = {12:1--12:34},
  year      = {2012},
  doi       = {10.1145/2379776.2379788}
}
@book{box2015time,
  title={Time series analysis: forecasting and control},
  author={Box, George EP and Jenkins, Gwilym M and Reinsel, Gregory C and Ljung, Greta M},
  year={2015},
  publisher={John Wiley \& Sons}
}
@article{makridakis2018statistical,
  title={Statistical and Machine Learning forecasting methods: Concerns and ways forward},
  author={Makridakis, Spyros and Spiliotis, Evangelos and Assimakopoulos, Vassilios},
  journal={PloS one},
  volume={13},
  number={3},
  year={2018},
  publisher={Public Library of Science}
}

@book{10.5555/574978,
author = {Box, George Edward Pelham and Jenkins, Gwilym},
title = {Time Series Analysis, Forecasting and Control},
year = {1990},
isbn = {0816211043},
publisher = {Holden-Day, Inc.},
address = {USA}
}


@book{yaffee2000introduction,
  title={An introduction to time series analysis and forecasting: with applications of SAS{\textregistered} and SPSS{\textregistered}},
  author={Yaffee, Robert Alan and McGee, Monnie},
  year={2000},
  publisher={Elsevier}
}
@article{milenkovic2018sarima,
  title={SARIMA modelling approach for railway passenger flow forecasting},
  author={Milenkovi{\'c}, Milo{\v{s}} and {\v{S}}vadlenka, Libor and Melichar, Vlastimil and Bojovi{\'c}, Neboj{\v{s}}a and Avramovi{\'c}, Zoran},
  journal={Transport},
  volume={33},
  number={5},
  pages={1113--1120},
  year={2018}
}

@article{wires-replay,
 author = "{W.M.P. van der} Aalst and A. Adriansyah and {B. van} Dongen",
 title = "{Replaying History on Process Models for Conformance Checking and Performance Analysis}",
 journal = {WIREs Data Mining and Knowledge Discovery},
 volume = {2},
 year = {2012},
 number = {2},
 pages = {182--192}}
 
 @inproceedings{SummerSimKeynote2018,
    author    = {W.M.P. van der Aalst},
  title= "{Process Mining and Simulation: A Match Made in Heaven!}",
  booktitle= "{Computer Simulation Conference}",

  publisher = {ACM Press},
  year= 2018,
  pages =  {1--12}}
  
  @article{ramsey1974characterization,
  title={Characterization of the partial autocorrelation function},
  author={Ramsey, Fred L and others},
  journal={The Annals of Statistics},
  volume={2},
  number={6},
  pages={1296--1301},
  year={1974},
  publisher={Institute of Mathematical Statistics}
}


@book{Pruyt-sd-book,
author = {Pruyt, Erik},
year = {2013},
month = {01},
title = {Small System Dynamics Models for Big Issues: Triple Jump towards Real-World Dynamic Complexity},
publisher= {TU Delft Library},
isbn = {9789461861955}
}


@article{DBLP:journals/is/AalstSS11,
  author    = {Wil M. P. van der Aalst and
               M. H. Schonenberg and
               Minseok Song},
  title     = {Time prediction based on process mining},
  journal   = {Inf. Syst.},
  volume    = {36},
  number    = {2},
  pages     = {450--475},
  year      = {2011},
  doi       = {10.1016/j.is.2010.09.001}
}

@inproceedings{DBLP:conf/caise/AalstPS10,
  author    = {Wil M. P. van der Aalst and
               Maja Pesic and
               Minseok Song},
  title     = {Beyond Process Mining: From the Past to Present and Future},
  booktitle = {Advanced Information Systems Engineering, 22nd International Conference,
               CAiSE 2010, Hammamet, Tunisia, June 7-9, 2010. Proceedings},
  pages     = {38--52},
  year      = {2010},
  doi       = {10.1007/978-3-642-13094-6\_5},
}

@article{DBLP:journals/tkde/AugustoCDRMMMS19,
  author    = {Adriano Augusto and
               Raffaele Conforti and
               Marlon Dumas and
               Marcello La Rosa and
               Fabrizio Maria Maggi and
               Andrea Marrella and
               Massimo Mecella and
               Allar Soo},
  title     = {Automated Discovery of Process Models from Event Logs: Review and
               Benchmark},
  journal   = {{IEEE} Trans. Knowl. Data Eng.},
  volume    = {31},
  number    = {4},
  pages     = {686--705},
  year      = {2019},
  doi       = {10.1109/TKDE.2018.2841877}
}


@inproceedings{DBLP:conf/apn/Westergaard13,
  author    = {Michael Westergaard},
  title     = {{CPN} Tools 4: Multi-formalism and Extensibility},
  booktitle = {Application and Theory of {P}etri Nets and Concurrency - 34th International
               Conference, {PETRI} {NETS} 2013, Milan, Italy, June 24-28, 2013. Proceedings},
  pages     = {400--409},
  year      = {2013},
  doi       = {10.1007/978-3-642-38697-8\_22}
}

@book{hamilton1994time,
  title={Time series analysis},
  author={Hamilton, James D},
  volume={2},
  year={1994},
  publisher={Princeton New Jersey}
}

@article{disc_sim_models_is,
author = "A. Rozinat and R.S. Mans and M. Song and {W.M.P. van der} Aalst",
title = "{Discovering Simulation Models}",
journal = {Information Systems},
volume = 34,
number = 3,
year = 2009,
pages = {305--327}}

@booklet{yawl-simulation-BPMcenter2008,
author = "A. Rozinat and M. Wynn and {W.M.P. van der} Aalst and {A.H.M. ter} Hofstede and C. Fidge",
title= "{Workflow Simulation for Operational Decision Support using YAWL and {P}ro{M}}",
year =  2008,
howpublished = {BPM Center Report BPM-08-04},
address = {BPMcenter.org}}

@article{sim-YAWL-ProM-dke,
author = "A. Rozinat and M. Wynn and {W.M.P. van der} Aalst and {A.H.M. ter} Hofstede and C. Fidge",
title= "{Workflow Simulation for Operational Decision Support}",
journal = {Data and Knowledge Engineering},
volume = 68,
number = 9,
year = 2009,
pages = {834--850}}

 @inproceedings{mahsaTimeseries,
  author    = {Mahsa Pourbafrani and       Sebastiaan J. van Zelst and  Wil M. P. van der Aalst},   title     = {Semi-Automated Time-Granularity Detection for Data-Driven Simulation Using Process Mining and System Dynamics},   booktitle = {Conceptual Modeling - 39th International Conference, {ER} 2020, Vienna,
               Austria, November 3-6, 2020, Proceedings},
                
      
               pages     = {},  
             
               year      = {2020},  
               doi       = {} }



@article{DBLP:journals/corr/abs-1910-05404,
  author    = {Manuel Camargo and
               Marlon Dumas and
               Oscar Gonz{\'{a}}lez Rojas},
  title     = {Automated Discovery of Business Process Simulation Models from Event
               Logs},
  journal   = {CoRR},
  volume    = {abs/1910.05404},
  year      = {2019},

  archivePrefix = {arXiv},
  eprint    = {1910.05404},
  timestamp = {Wed, 16 Oct 2019 16:25:53 +0200},
 
}
  %url       = {http://arxiv.org/abs/1910.05404},
 %biburl    = {https://dblp.org/rec/journals/corr/abs-1910-05404.bib},
  %bibsource = {dblp computer science bibliography, https://dblp.org}
  
  @article{DBLP:conf/bpm/CamargoDR19,
  author    = {Manuel Camargo and
               Marlon Dumas and
               Oscar Gonz{\'{a}}lez Rojas},
  title     = {Simod: a Tool for Automated Discovery of Business Process Simulation
               Models},
  booktitle = {Proceedings of Demonstration
               Track at {BPM} 2019},
  pages     = {139--143},
  year      = {2019},
}

@article{DBLP:journals/is/Rogge-SoltiW15,
  author    = {Andreas Rogge{-}Solti and Mathias Weske},
  title     = {Prediction of business process durations using non-Markovian stochastic {P}etri nets},
  journal   = {Inf. Syst.},
  volume    = {54},
  pages     = {1--14},
  year      = {2015},
  url       = {https://doi.org/10.1016/j.is.2015.04.004},
  doi       = {10.1016/j.is.2015.04.004},
  timestamp = {Wed, 14 Jun 2017 20:33:15 +0200},
  biburl    = {https://dblp.org/rec/journals/is/Rogge-SoltiW15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{VanDongen2005,
  Title                    = {The {P}ro{M} framework: A new era in process mining tool support},
  Author                   = {van Dongen, Boudewijn F and de Medeiros, Ana Karla A and Verbeek, HMW and Weijters, AJMM and van der Aalst, Wil M.P.},
  Booktitle                = {International Conference on Application and Theory of {P}etri Nets},
  Year                     = {2005},
  Organization             = {Springer},
  Pages                    = {444--454},

  Owner                    = {djr},
  Timestamp                = {2016.11.16}
}


@article{Rozina2008CPNdiscovery,
  author    = {Anne Rozinat and
               R. S. Mans and
               Minseok Song and
               Wil M. P. van der Aalst},
  title     = {Discovering colored Petri nets from event logs},
  journal   = {Int. J. Softw. Tools Technol. Transf.},
  volume    = {10},
  number    = {1},
  pages     = {57--74},
  year      = {2008},
  url       = {https://doi.org/10.1007/s10009-007-0051-0},
  doi       = {10.1007/s10009-007-0051-0},
  timestamp = {Thu, 02 Apr 2020 08:37:24 +0200},
  biburl    = {https://dblp.org/rec/journals/sttt/RozinatMSA08.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article {howcloseGawin,
      author = "Bartlomiej Gawin and Bartosz Marcinkowski",
      title = "How Close to Reality is the as-is Business Process Simulation Model?",
      journal = "Organizacija",
      year = "2015",
      publisher = "Sciendo",
      address = "Berlin",
      volume = "48",
      number = "3",
      doi = "https://doi.org/10.1515/orga-2015-0013",
      pages=      "155 - 175",
      url = "https://content.sciendo.com/view/journals/orga/48/3/article-p155.xml"
}



@article{DBLP:pm4py,
  author    = {Alessandro Berti and
               Sebastiaan J. van Zelst and
               Wil M. P. van der Aalst},
  title     = {Process Mining for Python (PM4Py): Bridging the Gap Between Process-
               and Data Science},
  journal   = {CoRR},
  volume    = {abs/1905.06169},
  year      = {2019},
  url       = {http://arxiv.org/abs/1905.06169},
  archivePrefix = {arXiv},
  eprint    = {1905.06169},
  timestamp = {Tue, 28 May 2019 12:48:08 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1905-06169.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/bpm/PufahlW17,
  author    = {Luise Pufahl and
               Mathias Weske},
  title     = {Extensible {BPMN} Process Simulator},
  booktitle = {Proceedings of the {BPM} Demo Track and {BPM} Dissertation Award co-located
               with 15th International Conference on Business Process Modeling (BPM)},
  year      = {2017},

  url       = {http://ceur-ws.org/Vol-1920/BPM\_2017\_paper\_198.pdf},
  timestamp = {Wed, 12 Feb 2020 16:44:57 +0100},
  biburl    = {https://dblp.org/rec/conf/bpm/PufahlW17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{MsimModelConstructionMartinDC16,
  author    = {Niels Martin and
               Beno{\^{\i}}t Depaire and
               An Caris},
  title     = {The Use of Process Mining in Business Process Simulation Model Construction
               - Structuring the Field},
  journal   = {Bus. Inf. Syst. Eng.},
  volume    = {58},
  number    = {1},
  pages     = {73--87},
  year      = {2016},
  url       = {https://doi.org/10.1007/s12599-015-0410-4},
  doi       = {10.1007/s12599-015-0410-4},
  timestamp = {Mon, 15 Jun 2020 16:57:30 +0200},
  biburl    = {https://dblp.org/rec/journals/bise/MartinDC16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{SPN,
author = {Baarir, Souheib and Beccuti, Marco and Cerotti, Davide and De Pierro, Massimiliano and Donatelli, Susanna and Franceschinis, Giuliana},
year = {2009},
month = {03},
pages = {4-9},
title = {The GreatSPN tool: recent enhancements},
volume = {36},
journal = {SIGMETRICS Performance Evaluation Review},
doi = {10.1145/1530873.1530876}
}

% reviewer points:
% Luise Pufahl, Mathias Weske: Extensible BPMN Process Simulator. BPM (Demos) 2017
%Martin, Niels, Benoît Depaire, and An Caris. "The use of process mining in business process simulation model construction." Business & Information Systems Engineering 58.1 (2016): 73-87.
%This paper describes a wide range of modeling tasks that exist when creating a realistic business process simulation model. As one can see, PMSIM currently ignores most of these modeling tasks. Hence, the validity of the produced simulation models and logs are unclear. PMSIM should either discover the necessary information from the event logs, ask the user to provide domain-knowledge or communicate which assumptions it makes.Finally, the current version of PMSIM makes some bizarre assumptions in the domain of process simulation. - The use of a normal distribution to model activity duration is remarkable and requires some mechanism to deal with negative durations (which are always possible). It is not clear how PMSIM deals with this. A triangular distribution would make more sense. - The use of a normal distribution to model inter-arrival time is also bizarre. Again, there is the issue of possible negative values that make no sense. Furthermore, it does not account for a long tail, which is very typical for these processes. An exponential distribution would be much more sensible here.


